A multidimensional measurement of photorealistic avatar quality of experience

Photorealistic avatars are human avatars that look, move, and talk like real people. The performance of photorealistic avatars has significantly improved recently based on objective metrics such as PSNR, SSIM, LPIPS, FID, and FVD. However, recent photorealistic avatar publications do not provide subjective tests of the avatars to measure human usability factors. We provide an open source test framework to subjectively measure photorealistic avatar performance in ten dimensions: realism, trust, comfortableness using, comfortableness interacting with, appropriateness for work, creepiness, formality, affinity, resemblance to the person, and emotion accuracy. Using telecommunication scenarios, we show that the correlation of nine of these subjective metrics with PSNR, SSIM, LPIPS, FID, and FVD is weak, and moderate for emotion accuracy. The crowdsourced subjective test framework is highly reproducible and accurate when compared to a panel of experts. We analyze a wide range of avatars from photorealistic to cartoon-like and show that some photorealistic avatars are approaching real video performance based on these dimensions. We also find that for avatars above a certain level of realism, eight of these measured dimensions are strongly correlated. This means that avatars that are not as realistic as real video will have lower trust, comfortableness using, comfortableness interacting with, appropriateness for work, formality, and affinity, and higher creepiness compared to real video. In addition, because there is a strong linear relationship between avatar affinity and realism, there is no uncanny valley effect for photorealistic avatars in the telecommunication scenario. We suggest several extensions of this test framework for future work and discuss design implications for telecommunication systems. The test framework is available at https://github.com/microsoft/P.910.

==> junk/boneyard.tex <==
\subsection{Standard deviation versus realism}
\begin{figure*}
    \centering
  \includegraphics[width=\columnwidth]{fig/NormalizedStd_vs_MOS_PerClip_Font20.png}
  \caption{Normalized Standard deviation versus MOS across each clip}
  \label{fig:NormalizedStd_vs_MOS_PerClip}
\end{figure*}

\begin{figure*}
    \centering
  \includegraphics[width=\columnwidth]{fig/NormalizedStd_vs_MOS_PerModel_Font20.png}
  \caption{Normalized Standard deviation versus MOS across each model}
  \label{fig:NormalizedStd_vs_MOS_PerModel}
\end{figure*}
\begin{table}
    \centering \includegraphics[width=0.5\columnwidth]{fig/MOSvsNormalizedStd.png}
    \caption{Average MOS across all dimensions versus Normalized Standard deviation across each model}
    \label{tab:MOSvsNormalizedStd}
\end{table}
\begin{table}
    \centering \includegraphics[width=0.5\linewidth]{fig/MOS_RealisticvsNormalizedStd.png}
    \caption{Realism versus Normalized Standard Deviation across each model}    \label{tab:MOS_RealisticVsNormalizedStd}
\end{table}
% Vishak
We observed that avatars with lower realism had higher relative variance in their MOS scores (e.g., avatars towards the right of the Figure \ref{fig:MOS_Scores_Model_AllAngles}a). To investigate this further we plot the Average MOS per item versus Normalized standard deviation defined as follows:
\begin{equation}
    \text{Normalized standard deviation} = \frac{\text{Standard deviation across items}}{\text{Average MOS across items}}
\end{equation}
We choose to normalize the standard deviation with the MOS to ensure a fair comparison of the variance across the avatars.
The plots shown in Figures \ref{fig:NormalizedStd_vs_MOS_PerClip} and \ref{fig:NormalizedStd_vs_MOS_PerModel} show that for the realistic clips where the MOS scores for the items are high, the normalized standard deviation is low. Table \ref{tab:MOSvsNormalizedStd} further highlights the clear distinction for MOS $\leq$ 2. A similar pattern can be observed in Table \ref{tab:MOS_RealisticVsNormalizedStd} where Realism scores are compared against the normalized standard deviation across all dimensions. We do this for both Average MOS across dimensions and for Realism to confirm the high correlations observed across dimensions shown in \ref{tab:PerModelCorrelation} also apply to the variance difference. The ``audio2photoreal\textunderscore0\textunderscore zoom'' avatar is a zoomed in version of the ``audio2photoreal'' avatar clip that masks the deformations in hands and torso. It can be seen that even after masking the issues like hands merging into each other, the avatar doesn't rate well due to unnatural lip and eye movements.

% I think it is too much to include both clip level and model level.
%\begin{figure}
%    \centering
%  \includegraphics[width=1\linewidth]{fig/PerClipCorrelation.png}
%  \caption{PCC for dimensions at clip level}
%  \label{fig:PerClipCorrelation}
%\end{figure}
